Large-Scale Bidirectional Training for Zero-Shot Image Captioning

When trained on large-scale datasets, image captioning models can understand the content of images from a general domain but often fail to generate accurate, detailed captions. To improve performance, pretraining-and-finetuning has been a key strategy for image captioning. However, we find that large-scale bidirectional training between image and text enables zero-shot image captioning. In this paper, we introduce Bidirectional Image Text Training in largER Scale, BITTERS, an efficient training and inference framework for zero-shot image captioning. We also propose a new evaluation benchmark which comprises of high quality datasets and an extensive set of metrics to properly evaluate zero-shot captioning accuracy and societal bias. We additionally provide an efficient finetuning approach for keyword extraction. We show that careful selection of large-scale training set and model architecture is the key to achieving zero-shot image captioning.

==> figures/adapter.tex <==
\begin{figure}[!tb]
  \centering
\includegraphics[width=0.97\linewidth]{figures/f_adapter.pdf}
\caption{Adapter for finetuning. Adapter is attached to each layer for parameter-efficient finetuning.
}
\label{adapter}
%\vspace{-4mm}
\end{figure}
